Eliminating Majority Illusion is Easy

Majority Illusion is a phenomenon in social networks wherein the decision by the majority of the network is not the same as one's personal social circle's majority, leading to an incorrect perception of the majority in a large network. In this paper, we present polynomial-time algorithms which can eliminate majority illusion in a network by altering as few connections as possible. Additionally, we prove that the more general problem of ensuring all neighbourhoods in the network are at least a $p$-fraction of the majority is NP-hard for most values of $p$.

==> polytope.tex <==
\section{Linear Program}
\subsection{Addition}
\begin{defn}
For the class of problems known as Eliminating Majority Illusion up to $p$ by adding edges, the function $d:B\cup R\rightarrow \mathcal{N} $ takes a node $v\in B\cup R$ and return the smallest non-negative integer $a$ such that $\frac{|N(v)\cap B|+a}{|N(v)|+a}\geq p$.
\end{defn}

\begin{defn}
For the class of problems known as Eliminating Majority Illusion up to $p$ by adding edges, the function $s:B\cup R\rightarrow \mathcal{N} $ takes a node $v\in B\cup R$ and return the largest non-negative integer  $a$ such that $\frac{|N(v)\cap B|}{|N(v)|+a}\geq p$, or $0$ if no such number exists.
\end{defn}

Observe that, for any node $v\in B\cup R$, at least one of 
$s(v)$ and $d(v)$ is zero.

We now construct a linear program that will solve the
(Fact-Checking problem), (Anti-Insurrection of $\frac{k}{n}$ problem) addition problem.\todo{Come up with nice names for these problems.} To do this, take $G=(B\cup R, E)$ and let $N_E(v)=v\cup \{u: (u,v)\in E\}$
be the neighbourhood of $v$, including $v$ itself.

Given $G=(B\cup R, E)$ we define an auxiliary graph $G^*=(B\cup R, E^*)$, called the {\em availability graph}. Its edges are 
the edges in the complement of $G$ excluding those between two red nodes. That is, $E^*$ = $\overline{E}(R,B) \cup \overline{E}(G[B])$. Now let 
    $$
    w_e =
    \begin{cases}
    \frac{1}{1-p} &\mathrm{if}\ e \in \overline{E}(R,B)\\
    \frac1p &\mathrm{if}\ e \in \overline{E}(G[B])
    \end{cases}
    $$
and
      $$
   b^*(v) =
    \begin{cases}
k\cdot d(v) &\mathrm{if}\ v \in R \\
(n-k)\cdot|N_{E^*}(v)\cap B|- (n-k)\cdot d(v)+k\cdot s(v) &\mathrm{if}\ v \in B
    \end{cases}
    $$



We may now define an integer program.
\begin{equation}\label{addIP}
\begin{array}{lrl@{}ll}
\text{maximize}  &    \displaystyle\sum\limits_{e\in E^*} w_e \cdot x_e & &\\
\text{subject to}\\
  & \displaystyle\sum\limits_{e:e \in \delta(v)}   w_e\cdot x_e  &= b^*(v)  &v\in R(G^*)\\
  & \displaystyle\sum\limits_{e:e \in \delta(v)}   w_e \cdot x_e  &\leq b^*(v)  &v\in B(G^*)\\
 \displaystyle\sum\limits_{e:e \in E^*(G^*[X])}w_e \cdot x_e  &+\displaystyle\sum\limits_{e:e \in F}    w_e\cdot x_e &\leq \Bigl\lfloor \frac12\Bigl(\displaystyle\sum\limits_{v:v \in X}b^*(v)+ \displaystyle\sum\limits_{e:e \in F}w_e\Bigr) \Bigr\rfloor  ~& \begin{array}{l}
\forall X\subseteq B\cup R\\
\forall F \subseteq \delta(X)
\end{array} \\
&    x_e &\in \{0,1\} &e\in E^*(G^*)
\end{array}
\end{equation}

\begin{thm}
    The integer program~(\ref{addIP}) is the addition problem.
\end{thm}

\begin{proof}

    \begin{claim}
        An optimal solution $y$ to the addition problem is a feasible solution to the integer program~(\ref{addIP})
    \end{claim}

    \begin{proof}
        
    

    Firstly, note $y\in \{0,1\}^{E^*}$, because any edge in  $\overline{E}(G[R])$ can be removed from $y$ without negatively impacting any node, contradicting optimality.

    Secondly, note that for each node $v \in R$, we have $$\displaystyle\sum\limits_{u:u \in N_{E^*}(v)\cap B}   y_{uv}  = d(v)$$
    
    The reason is each such $v$ needs at least $d(v)$ new neighbours in $B$ to eliminate illusion. Each $v$ also needs at most $d(v)$ new neighbours, otherwise we can delete an incident edge while still eliminating illusion, contradicting optimality. Multiplying both sides by $k$ gives

$$k\cdot \displaystyle\sum\limits_{u:u \in N_{E^*}(v)\cap B} y_{uv}  = k\cdot d(v) = b^*(v)$$

    Thirdly, note that for each $v \in B$, we have 
    
    $$k\cdot\Bigl(\displaystyle\sum\limits_{u:u\in N_{E^*}(v) \cap R} y_{uv}-s(v)\Bigr) \leq (n-k)\cdot\Bigl(\displaystyle\sum\limits_{u:u \in N_{E^*}(v)\cap B} y_{uv}-d(v)\Bigr) $$
    
    The reason is each such $v$ needs at least $k$ nodes in $B$ for every $n-k$ nodes in $R$. Therefore the total number of new neighbours in $B$, minus the deficit of $v$, $d(v)$, muliplied by $n-k$, should exceed the total number of new nighbours in $R$, minus the surplus of $v$, $s(v)$, multiplied by $k$. 

    Rearranging gives

    $$(n-k)\cdot\Bigl(\displaystyle\sum\limits_{u:u \in N_{E^*}(v)\cap B} -y_{uv}\Bigr) + k\cdot\Bigl(\displaystyle\sum\limits_{u:u\in N_{E^*}(v) \cap R} y_{uv}\Bigr) \leq -(n-k)\cdot d(v) + k\cdot s(v)$$

    then, we can add $|N_{E^*}(v)\cap B|$ to both sides o obtain

    $$(n-k)\cdot\Bigl(\displaystyle\sum\limits_{u:u \in N_{E^*}(v)\cap B}1 -y_{uv}\Bigr) + k\cdot\Bigl(\displaystyle\sum\limits_{u:u\in N_{E^*}(v) \cap R} y_{uv}\Bigr) \leq b^*(v)$$

    Lastly, for every $X\subseteq B\cup R$, and every $F \subseteq \delta_{E^*}(X)$, we have 

\begin{eqnarray*}
  \displaystyle\sum\limits_{v:v \in X}b^*(v) &=& 2(n-k)\cdot\Bigl(\displaystyle\sum\limits_{uv:u,v \in X\cap B}1 -y_{uv}\Bigr) + 2k\cdot\Bigl(\displaystyle\sum\limits_{uv:u\in X\cap B, v \in X\cap R} y_{uv}\Bigr)+ \\
&&(n-k)\cdot\Bigl(\displaystyle\sum\limits_{uv:u\in X\cap B, v \in B\setminus X}1- y_{uv}\Bigr)+ 
k\cdot\Bigl(\displaystyle\sum\limits_{uv:u\in X\cap B, v \in R\setminus X} y_{uv}\Bigr) +
k\cdot\Bigl(\displaystyle\sum\limits_{uv:u\in X\cap R, v \in B\setminus X}y_{uv}\Bigr) \\
&\geq& 2(n-k)\cdot\Bigl(\displaystyle\sum\limits_{e:e \in E^*(G^*[B])\cap E^*(G^*[X])}1 -y_{uv}\Bigr) + 2k\cdot\Bigl(\displaystyle\sum\limits_{e:e \in E^*(G^*[B])\cap E^*(R,B)} y_{uv}\Bigr)+ \\
&&(n-k)\cdot\displaystyle\sum\limits_{
e:e \in E^*(G^*[B])\cap F}(1-y_e)+ k\cdot\displaystyle\sum\limits_{
e:e \in E^*(R,B)\cap F
}y_e 
\end{eqnarray*}

Also, we have

$$(n-k)\cdot\displaystyle\sum\limits_{
e:e \in E^*(G^*[B])\cap F}(1-y_e)+ k\cdot\displaystyle\sum\limits_{
e:e \in E^*(R,B)\cap F
}y_e \leq \displaystyle\sum\limits_{
e:e \in E^*(G^*[B])\cap F}(n-k)+ \displaystyle\sum\limits_{
e:e \in E^*(R,B)\cap F
}k $$

thus we can sum these two inequalities to obtain

$$
2(n-k)\cdot\displaystyle\sum\limits_{\substack{
e:e \in E^*(G^*[B])\\
e \in E^*(G^*[X])\cup F}}(1-y_e)+ 2k\cdot\displaystyle\sum\limits_{\substack{
e:e \in E^*(R,B)\\
e \in E^*(G^*[X])\cup F
}}y_e \leq \displaystyle\sum\limits_{v:v \in X}b^*(v)+ \displaystyle\sum\limits_{\substack{e:e \in F \\e \in E^*(G^*[B])}}n-k +\displaystyle\sum\limits_{\substack{e:e \in F \\e \in E^*(R,B)}}k $$ 

By if we divide both sides by 2, and take the floor of both sides, then by integrality of $y$ we get

$$
(n-k)\cdot\displaystyle\sum\limits_{\substack{
e:e \in E^*(G^*[B])\\
e \in E^*(G^*[X])\cup F}}(1-y_e)+ k\cdot\displaystyle\sum\limits_{\substack{
e:e \in E^*(R,B)\\
e \in E^*(G^*[X])\cup F
}}y_e \leq \Bigl\lfloor \frac12\Bigl(\displaystyle\sum\limits_{v:v \in X}b^*(v)+ \displaystyle\sum\limits_{\substack{e:e \in F \\e \in E^*(G^*[B])}}n-k +\displaystyle\sum\limits_{\substack{e:e \in F \\e \in E^*(R,B)}}k \Bigr) \Bigr\rfloor $$ 

\end{proof}

\begin{claim}
    An optimal solution $y$ to the integer program~(\ref{addIP}) is a feasible solution to the addition problem.
\end{claim}

\begin{proof}
    Firstly, note that for each node $v \in R$, we have $$k\cdot\displaystyle\sum\limits_{u:u \in N_{E^*}(v)\cap B}   y_{uv}  = b^*(v)$$.

    This simplifies to 

    $$\displaystyle\sum\limits_{u:u \in N_{E^*}(v)\cap B}   y_{uv}  = d(v)$$

    Thus $y$ will eliminate majority illision in each such node $v \in R$ because it connects $v$ to exactly $d(v)$ blue nodes and no additional red nodes.

    Lastly, note that for each $v \in B$, we have 

    $$(n-k)\cdot\Bigl(\displaystyle\sum\limits_{u:u \in N_{E^*}(v)\cap B}1 -y_{uv}\Bigr) + k\cdot\Bigl(\displaystyle\sum\limits_{u:u\in N_{E^*}(v) \cap R} y_{uv}\Bigr) \leq b^*(v)$$

    if we subtract $|N_{E^*}(v)\cap B|$ from both sides we obtain

    $$(n-k)\cdot\Bigl(\displaystyle\sum\limits_{u:u \in N_{E^*}(v)\cap B} -y_{uv}\Bigr) + k\cdot\Bigl(\displaystyle\sum\limits_{u:u\in N_{E^*}(v) \cap R} y_{uv}\Bigr) \leq -(n-k)\cdot d(v) + k\cdot s(v)$$

    then by rearranging we have
    $$k\cdot\Bigl(\displaystyle\sum\limits_{u:u\in N_{E^*}(v) \cap R} y_{uv}-s(v)\Bigr) \leq (n-k)\cdot\Bigl(\displaystyle\sum\limits_{u:u \in N_{E^*}(v)\cap B} y_{uv}-d(v)\Bigr) $$

    Therefore the total number of new neighbours in $B$, minus the deficit of $v$, $d(v)$, multiplied by $n-k$, exceeds the total number of new neighbours in $R$, minus the surplus of $v$, $s(v)$, multiplied by $k$. This means illusion is eliminated for any such $v \in B$ 

\end{proof}

Finally, it remains to show that the two problems have the same optimal solutions. In both cases, only edges of $E^*$ are used in an optimal solution, and exactly $\displaystyle\sum\limits_{u:u \in R} d(u)$ edges in $E^*(R,B)$ are used in both cases. Thus the integer program \ref{addIP}is maximizing the term $(n-k)\cdot\displaystyle\sum\limits_{e\in E^*(G^*[B])} -y_e$ as the rest of its objective function is constant, while the addition problem is minimizing the number of edges used within $E^*(G^*[B])$ as the number of other edges is constant. The two are therefore equivalent because maximizing the term $(n-k)\cdot\displaystyle\sum\limits_{e\in E^*(G^*[B])} -y_e$ is equivalent to minimizing the term $\displaystyle\sum\limits_{e\in E^*(G^*[B])} y_e$.
\end{proof}

Now, in order to solve the addition problem, we can use integer program \ref{addIP}. In fact, we will show that the addition problem is solvable in polynomial time by proving the linear relaxation of integer program \ref{addIP} is totally dual integral and solvable in polynomial time. To do so, we need the following.




We now have three tasks to complete. First, we must show that the integer program~(\ref{addIP}) is the addition problem.
Second we must prove that its linear program relaxation is
integral. Thirdly, we must show the linear program relaxation can be solved in polynomial time, despite the fact there are an exponential number of constraints.


To accomplish the first task, let's apply the following change of variables.
$$
    y_e =
    \begin{cases}
    x_e &\mathrm{if}\ e \in E^*(R,B)\\
    1-x_e &\mathrm{if}\ e \in E^*(G^*[B])
    \end{cases}
$$

let $p = \frac{k}{n}$
This induces the following integer program.
\begin{eqnarray*}\label{addIP-y}
\text{maximize} \ \hspace{6cm}\  \\
\\
(n-k)\cdot\displaystyle\sum\limits_{e\in E^*(G^*[B])} (1-y_e) + k\cdot\displaystyle\sum\limits_{e\in E^*(R,B)}y_e&&\\
\\
\text{subject to} \ \hspace{6cm}\ &\\
\\
  k\cdot\displaystyle\sum\limits_{u:u \in N_{E^*}(v)\cap B}   y_{uv}  &=& b^*(v)  \qquad  v\in R(G^*)\\
   (n-k)\cdot\displaystyle\sum\limits_{u:u \in N_{E^*}(v)\cap B}   (1-y_{uv})  +k\cdot\displaystyle\sum\limits_{u:u\in N_{E^*}(v) \cap R}    y_{uv} &\leq& b^*(v)  \qquad v\in B(G^*)\\
(n-k)\cdot\displaystyle\sum\limits_{\substack{
e:e \in E^*(G^*[B])\\
e \in E^*(G^*[X])\cup F}}(1-y_e)+ k\cdot\displaystyle\sum\limits_{\substack{
e:e \in E^*(R,B)\\
e \in E^*(G^*[X])\cup F
}}y_e &\leq& \Bigl\lfloor \frac12\Bigl(\displaystyle\sum\limits_{v:v \in X}b^*(v)+ \displaystyle\sum\limits_{\substack{e:e \in F \\e \in E^*(G^*[B])}}n-k +\displaystyle\sum\limits_{\substack{e:e \in F \\e \in E^*(R,B)}}k \Bigr) \Bigr\rfloor   \\
&& \forall X\subseteq B\cup R, ~ \forall F \subseteq \delta_{E^*}(X)\\
    y_e &\in& \{0,1\} \qquad e\in E^*(G^*)
\end{eqnarray*}
\todo[inline]{Explain steps above and transform $X,F$ constraints to $y_e$s.}


\begin{claim}\label{addclaim}
$x$ is a solution to IP~(\ref{addIP}) if and only if
$y$ is a solution to the original Eliminating illusion instance containing exactly $\sum\limits_{v:v \in R}d(v)$ edges of $E^*(R,B)$.
\end{claim}   

    \begin{proof}
 The constraints imply that, for all $v \in R$,
  $$\sum\limits_{e:e\in \delta_{E^*}(v)} \frac{1}{1-p}\cdot y_e = \sum\limits_{e:e\in \delta_{E^*}(v)} w_e \cdot y_e = b^*(v) =\frac{1}{1-p}\cdot d(v)$$
 \todo[inline]{I don't understand the last equality as the definition above is $b^*(v)=\frac{1}{p}\cdot d(v)$ for red nodes.}

 It follows that $y$ eliminates illusion for each red node using exactly $\sum\limits_{v:v \in R}d(v)$ edges of $E^*(R,B)$
 because
$$\sum\limits_{e:e\in \delta_{E^*}(v)} y_e = d(v)$$

Next take any blue node $v \in B$. Consider the corresponding inequality:

\begin{eqnarray*}
    \displaystyle\sum\limits_{e:e \in \delta(v)\cap E^*(G^*[B])}   w_e \cdot (1-y_e)  +\displaystyle\sum\limits_{e:e \in \delta(v)\cap E^*(R,B)}   w_e \cdot y_e &\leq& b^*(v) \\
\end{eqnarray*}

If we subtract $\frac1p\cdot|N_{E^*}(v)\cap B|$ from both sides, then by the definition of $b^*(v)$ we obtain:

\begin{eqnarray*}
    \displaystyle\sum\limits_{e:e \in \delta(v)\cap E^*(G^*[B])}   -w_e \cdot y_e  +\displaystyle\sum\limits_{e:e \in \delta(v)\cap E^*(R,B)}   w_e \cdot y_e &\leq& - \frac1p\cdot d(v)+\frac{1}{1-p}\cdot s(v) \\
\end{eqnarray*}

Rearranging and substituting the definition of $w_e$, we obtain:

\begin{eqnarray*}
      \frac{1}{1-p}\cdot\Bigl[\bigl(\displaystyle\sum\limits_{e:e \in \delta(v)\cap E^*(R,B)} y_e \bigr) - s(v)\Bigr]&\leq& \frac1p\cdot\Bigl[\bigl(\displaystyle\sum\limits_{e:e \in \delta(v)\cap E^*(G^*[B])}y(e)\bigr) - d(v)\Bigr] \\
\end{eqnarray*}

\begin{eqnarray*}
b^*(v) &=& \frac1p\cdot|N_{E^*}(v)\cap B|- \frac1p\cdot d(v)+\frac{1}{1-p}\cdot s(v)\\
&\ge& \sum_{e:e \in \delta(v)\cap E^*(G^*[B])}   w_e \cdot (1-y_e)  +\sum_{e:e \in \delta(v)\cap E^*(R,B)}   w_e \cdot y_e  \\
&=& \frac{1}{p}\cdot \sum_{e:e \in \delta(v)\cap E^*(G^*[B])}    (1-y_e)  + \frac{1}{1-p}\cdot \sum_{e:e \in \delta(v)\cap E^*(R,B)}   y_e 
 \end{eqnarray*}
Rearranging we obtain
\begin{eqnarray*}
\frac1p\cdot d(v)-\frac{1}{1-p}\cdot s(v)
 + \frac{1}{1-p}\cdot \sum_{e:e \in \delta(v)\cap E^*(R,B)}   y_e 
&\le&
\frac1p\cdot|N_{E^*}(v)\cap B|- \frac{1}{p}\cdot \sum_{e:e \in \delta(v)\cap E^*(G^*[B])}    (1-y_e) \\
&=&
 \frac{1}{p}\cdot \sum_{e:e \in \delta(v)\cap E^*(G^*[B])} y_e
 \end{eqnarray*}
But this is true if and only if
\begin{eqnarray*}
\frac1p\cdot d(v)-\frac{1}{1-p}\cdot s(v)
 + \frac{1}{1-p}\cdot \sum_{e:e \in \delta(v)\cap E^*(R,B)}   x_e 
&=&
 \frac{1}{p}\cdot \sum_{e:e \in \delta(v)\cap E^*(G^*[B])} (1-x_e)\\
 &=&
 \frac{1}{p}\cdot |N_{E^*}(v)\cap B|
 - \frac{1}{p}\cdot \sum_{e:e \in \delta(v)\cap E^*(G^*[B])} x_e
 \end{eqnarray*}
Thus
\begin{eqnarray*}
b^*(v)&=&  \frac{1}{p}\cdot |N_{E^*}(v)\cap B|
-\frac1p\cdot d(v)+\frac{1}{1-p}\cdot s(v)\\
&\ge&
\frac{1}{1-p}\cdot \sum_{e:e \in \delta(v)\cap E^*(R,B)}   x_e 
+ \frac{1}{p}\cdot \sum_{e:e \in \delta(v)\cap E^*(G^*[B])} x_e\\
&=& \sum\limits_{e:e\in \delta_{E^*}(v)} w_e\cdot x_e
 \end{eqnarray*}

    This implies that $y$ eliminates illusion for each $v \in B$ if and only if, for all $v \in B$, 
    $$b^*(v) \ge \sum\limits_{e:e\in \delta_{E^*}(v)} w_e\cdot x_e
  $$   
  \todo[inline]{why is this what we need? Also, what about the X,F constraints, how do we know they don't mess things up, e.g. by making it infeasible?}
  \end{proof}




\begin{thm}
    An instance of Eliminating illusion to at least $p$ percent by adding edges for graph $G=(B\cup R, E)$ reduces to an instance of LP \ref{addLP} in polynomial time
\end{thm}
\begin{proof}
  
    What remains to be proven is, if $x,y$ are as in claim \ref{addclaim}, and if $x$ is optimal, then $y$ is eliminates illusion optimally. By theorem \ref{addTDI}, if $x$ is an optimal solution to LP \ref{addLP}, it is integral. Therefore, $y$ is also integral by definition. 
    
    Firstly, note that any set of edges which eliminates illusion optimally uses no edges of $\overline{E}(G[R])$ and exactly $\sum\limits_{v:v \in R}d(v)$ edges of $\overline{E}(R,B)$. This is the case because in order to eliminate illusion from $v \in R$, $d(v)$ edges incident to $v$ are required at minimum by definition. If any edges of $\overline{E}(G[R])$ have been added incident to $v$, they can be deleted without increasing illusion, contradicting optimality. Similarly, if more than $d(v)$ edges of $\overline{E}(R,B)$ have been added, they can be deleted without increasing illusion, contradicting optimality. 

    Therefore showing that $y$ is optimal amounts to showing that $y$ uses the minimum number of edges in $\overline{E}(G[B])$. However, this is equivalent to $y$ avoiding the maximum number of edges in $\overline{E}(G[B])$. By the definition of $y$ and $x$, this equates to $x$ using the maximum number of edges in $\overline{E}(G[B])$. However, this is exactly what $x$ does, because $x$ maximizes $$w\cdot x = \frac1p\cdot\sum\limits_{v:v \in R}\cdot d(v) + \frac{1}{1-p}\cdot \sum\limits_{e:e\in\overline{E}(G^*[B])} x_e$$ Thus, $y$ is optimal.
\end{proof}


\begin{thm}\label{addTDI}
    LP \ref{addLP} is TDI
\end{thm}

\begin{proof}
    This is the weighted $b$-matching LP for $G^*$ and unit edge capacities, altered repeatedly by swapping an inequality for an equality.\todo{Add Reference.} The standard weighted  b-matching LP for $G^*$ and unit edge capacities is TDI, and swapping an inequality for an equality preserves TDI.\todo{Add Reference.}

\todo[inline]{Break this proofinto parts. Present the generic b-matching LP. The rewrite and expand the LP in terms of R/B nodes. Then explain the changes from inequalies to equalities. Before arriving at the LP we wanted.}

    \begin{equation}\label{addLP}
\begin{array}{lrl@{}ll}
\text{maximize}  &    \displaystyle\sum\limits_{e\in E^*} w_e \cdot x_e & &\\
\text{subject to} & x_e &\leq 1  &e\in E^*(G^*)\\
  & \displaystyle\sum\limits_{e:e \in \delta(v)}   w_e\cdot x_e  &= b^*(v)  &v\in R(G^*)\\
  & \displaystyle\sum\limits_{e:e \in \delta(v)}   w_e \cdot x_e  &\leq b^*(v)  &v\in B(G^*)\\
 \displaystyle\sum\limits_{e:e \in E^*(G^*[X])}w_e \cdot x_e  &+\displaystyle\sum\limits_{e:e \in F}    w_e\cdot x_e &\leq \Bigl\lfloor \frac12\Bigl(\displaystyle\sum\limits_{v:v \in X}b^*(v)+ \displaystyle\sum\limits_{e:e \in F}w_e\Bigr) \Bigr\rfloor  ~& \begin{array}{l}
X\subseteq B\cup R\\
F \subseteq \delta(X)
\end{array} \\
&    x_e &\ge 0 &e\in E^*(G^*)
\end{array}
\end{equation}
\end{proof}



\subsection{Removal}

\begin{defn}
For the class of problems known as Eliminating Majority Illusion up to $p$ by removing edges, the function $d:B\cup R\rightarrow \mathcal{N} $ takes a node $v\in B\cup R$ and return the smallest non-negative integer  $r$ such that $\frac{|N(v)\cap B|}{|N(v)|-r}\geq p$.
\end{defn}

\begin{defn}
For the class of problems known as Eliminating Majority Illusion up to $p$ by removing edges, the function $s:B\cup R\rightarrow \mathcal{N} $ takes a node $v\in B\cup R$ and return the largest non-negative integer  $r$ such that $\frac{|N(v)\cap B|-r}{|N(v)|-r}\geq p$, or $0$ if no such number exists.
\end{defn}



\begin{equation}\label{removeLP}
\begin{array}{llrl@{}ll}
\text{maximize}  &   & w \cdot x & &\\
\text{subject to} & &x_e &\leq 1,  &e\in E^*(G^*)\\
  & \displaystyle\sum\limits_{e:e \in \delta(v)}   &w_e\cdot x_e  &= b^*(v),  &v\in B(G^*)\\
  & \displaystyle\sum\limits_{e:e \in \delta(v)}   &w_e \cdot x_e  &\leq b^*(v),  &v\in R(G^*)\\
 \displaystyle\sum\limits_{e:e \in E^*(G^*[X])}w_e \cdot x_e  &+\displaystyle\sum\limits_{e:e \in F}   & w_e\cdot x_e &\leq \Bigl\lfloor \frac12\Bigl(\displaystyle\sum\limits_{v:v \in X}b^*(v)+ \displaystyle\sum\limits_{e:e \in F}w_e\Bigr) \Bigr\rfloor  ~& \begin{array}{l}
X\subseteq B\cup R\\
F \subseteq \delta(X)
\end{array} \\
&  &   x_e &\geq 0, &e\in E^*
\end{array}
\end{equation}

\begin{cor}\label{removeTDI}
    LP \ref{removeLP} is TDI
\end{cor}

\begin{thm}
    An instance of Eliminating illusion to at least $p$ percent by removing edges for graph $G=(B\cup R, E)$ reduces to an instance of LP \ref{removeLP} in polynomial time
\end{thm}

\begin{proof}
    Begin by constructing $G^*= (B\cup R, E^*)$ from $G$ in the following way. Let $E^*$ = $E(R,B) \cup E(G[R])$. Let $w_e = \frac1p$ for $e \in E(R,B)$ and $w_e = \frac{1}{1-p}$ for $e \in G[R]$ Let $b^*(v) = \frac1p\cdot d(v)$ for $v \in B$ and $b^*(v) = \frac{1}{1-p}|N_{E^*}(v)\cap R|- \frac{1}{1-p}\cdot d(v)+\frac1p\cdot s(v)$ for $v \in R$. 
    
    \claim{Let $x,y\in \{0,1\}^{E^*}$, where $x_e=y_e$ for  $e\in E^*(R,B)$ and $x_e = 1-y_e$ for $e\in E^*(G^*[R])$. $x$ is a solution to LP \ref{removeLP} with the above parameters if and only if $y$ is a solution to the original Eliminating illusion instance removing exactly $\sum\limits_{v:v \in B}d(v)$ edges of $E^*(R,B)$.}\label{removeclaim}
    
    \begin{proof}
    First note that by definition $y$ eliminates illusion for each $v \in B$ using exactly $\sum\limits_{v:v \in B}d(v)$ edges of $E^*(R,B)$ if and only if, for all $v \in B$, 
    
    $$\sum\limits_{e:e\in \delta_{E^*}(v)} \frac1p y_e = \sum\limits_{e:e\in \delta_{E^*}(v)} w_e \cdot x_e = \frac1p\cdot d(v) = b^*(v)$$

    Next note that by definition $y$ eliminates illusion for each $v \in R$ if and only if, for all $v \in R$,
    
    $$\sum\limits_{uv:uv\in E^*, u \in R} \frac{1}{1-p}
    \cdot y_{uv}\geq \frac{1}{1-p}
    \cdot d(v)-\frac1p\cdot s(v) + \sum\limits_{uv:uv\in E^*, u \in B} \frac1p\cdot y_{uv}$$

    This implies that $y$ eliminates illusion for each $v \in R$ if and only if, for all $v \in R$,
    
    $$\sum\limits_{uv:uv\in E^*, u \in R} \frac{1}{1-p}
    \cdot (1-x_{uv}) \geq \frac{1}{1-p}
    \cdot d(v)-\frac1p\cdot s(v) + \sum\limits_{uv:uv\in E^*, u \in B} \frac1p\cdot x_{uv}$$
    
    or, equivalently,
    
    \begin{equation}
    \begin{array}{r@{}l}
    b^*(v) &= \frac{1}{1-p}\cdot |N_{E^*}(v)\cap R| -\frac{1}{1-p}\cdot d(v) + \frac1p\cdot s(v)\\
    &\geq  \sum\limits_{uv:uv\in E^*, u \in B} \frac{1}{1-p}
    \cdot x_{uv} + \sum\limits_{uv:uv\in E^*, u \in R} \frac1p\cdot x_{uv}\\
    &=\sum\limits_{e:e\in \delta_{E^*}(v)} w_e\cdot x_e
    \end{array}
    \end{equation}
    
    \end{proof}

    What remains to be proven is, if $x,y$ are as in claim \ref{addclaim}, and if $x$ is optimal, then $y$ is eliminates illusion optimally. By corollary \ref{removeTDI}, if $x$ is an optimal solution to LP \ref{removeLP}, it is integral. Therefore, $y$ is also integral by definition. 
    
    Firstly, note that any set of edges which eliminates illusion optimally uses no edges of $E(G[B])$ and exactly $\sum\limits_{v:v \in B}d(v)$ edges of $E(R,B)$. This is the case because in order to eliminate illusion from $v \in B$, $d(v)$ edges incident to $v$ are removed at minimum by definition. If any edges of $E(G[R])$ have been remove incident to $v$, they can be re-added without increasing illusion, contradicting optimality. Similarly, if more than $d(v)$ edges of $E(R,B)$ have been removed, they can be re-added without increasing illusion, contradicting optimality. 

    Therefore showing that $y$ is optimal amounts to showing that $y$ uses the minimum number of edges in $E(G[R])$. However, this is equivalent to $y$ avoiding the maximum number of edges in $E(G[R])$. By the definition of $y$ and $x$, this equates to $x$ using the maximum number of edges in $E(G[R])$. However, this is exactly what $x$ does, because $x$ maximizes $$w\cdot x = \frac1p\cdot\sum\limits_{v:v \in B}\cdot d(v) + \frac{1}{1-p}\cdot \sum\limits_{e:E(G[R])} x_e$$. Thus, $y$ is optimal.
\end{proof}

